Robust RL with LLM-Driven Data Synthesis and Policy Adaptation for Autonomous Driving

The integration of Large Language Models (LLMs) into autonomous driving systems demonstrates strong common sense and reasoning abilities, effectively addressing the pitfalls of purely data-driven methods. Current LLM-based agents require lengthy inference times and face challenges in interacting with real-time autonomous driving environments. A key open question is whether we can effectively leverage the knowledge from LLMs to train an efficient and robust Reinforcement Learning (RL) agent. This paper introduces RAPID, a novel \underline{\textbf{R}}obust \underline{\textbf{A}}daptive \underline{\textbf{P}}olicy \underline{\textbf{I}}nfusion and \underline{\textbf{D}}istillation framework, which trains specialized mix-of-policy RL agents using data synthesized by an LLM-based driving agent and online adaptation. RAPID features three key designs: 1) utilization of offline data collected from an LLM agent to distil expert knowledge into RL policies for faster real-time inference; 2) introduction of robust distillation in RL to inherit both performance and robustness from LLM-based teacher; and 3) employment of a mix-of-policy approach for joint decision decoding with a policy adapter. Through fine-tuning via online environment interaction, RAPID reduces the forgetting of LLM knowledge while maintaining adaptability to different tasks. Extensive experiments demonstrate RAPID's capability to effectively integrate LLM knowledge into scaled-down RL policies in an efficient, adaptable, and robust way. Code and checkpoints will be made publicly available upon acceptance.

==> algorithm/algorithm_1.tex <==
\begin{algorithm}[tb]
\caption{Semi-Contrastive Adversarial Augmentation}
\textbf{Require:} Offline dataset $\mathcal{D}$,  learning rate $\alpha$, training steps $T$\\
\textbf{Initialisation:} Critic function $\varrho(\cdot)$, policy function $\varphi(\psi(\cdot))$
\begin{algorithmic}[1]
% \State Randomly initialise value function $V_{\theta}$, and policy function $\pi_{\phi}$
\For {training timestep $1\dots T$}
\State Sample a mini-batch from the offline dataset:

$(s_t^i, a_t^i, s_{t+1}^i, g^i) \sim \mathcal{D}$
% \State Apply data augmentation and encode $h_t\leftarrow f_{\xi}(s_t, g)$
\State Construct negative tuples:

$\left<s_t^i,g^i\right>^{-}$ and $\left<s_{t+1}^i,g^i\right>^{-}$
\State Compute the semi-contrastive augmented samples:

$\mathcal{V}_{scr}(s_t^i)$ and $\mathcal{V}_{scr}(g^i)$ by 
% $\hat{s}_t^i = \mathcal{SCAA}(s_t^i)$, $\hat{s}_{t+1}^i = \mathcal{SCAA}(s_{t+1}^i)$
\State 
    Augment critic value:
    
    $\hat{\varrho} \gets \mathbb{E} [\varrho(s_{t}^i,g^i,a_t^i) + \varrho(\mathcal{V}_{scr}(s_{t}^i),\mathcal{V}_{scr}(g^i),a_t^i)]$
\State Augment actor value:

$\scriptstyle\hat{\varphi} \gets \mathbb{E}[\varphi(\psi(\left<s_t^i, g^i\right>)) + \varphi(\psi(\left<\mathcal{V}_{scr}(s_{t}^i), \mathcal{V}_{scr}(g^i)\right>)]$
\State Update encoder weights: 
$\scriptstyle\theta_{\psi} \gets \theta_\psi - \alpha \nabla \mathcal{L}_\psi(\left<s_t^i,g^i\right>)$
\State Update actor weights:
$\theta_\varphi \gets \theta_\varphi - \alpha \nabla \mathcal{L}_\varphi(\hat{\varphi})$
\State Update critic weights: 
$\theta_\varrho\gets \theta_\varrho-\alpha  \nabla \mathcal{L}_\varrho(\hat{\varrho})$
\EndFor
\end{algorithmic}
\label{algorithm_scaa}
\end{algorithm}

==> tables/distil_results.tex <==
\begin{tabular}{@{}cc|cc|cc|cc@{}}
\toprule
\multicolumn{2}{c|}{Methods}          & \multicolumn{2}{c|}{\textsc{lane-4-density-2}}   & \multicolumn{2}{c|}{\textsc{lane-5-density-2.5}} & \multicolumn{2}{c}{\textsc{lane-5-density-3}} \\ 
&  &rewards &safety &rewards &safety &rewards &safety \\
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{GPT-3.5}}  
& \multicolumn{1}{c|}{online DQN}     
& 12.48$_{\pm 8.56}$   &  14.38$_{\pm 1.57}$   &  12.87$_{\pm 9.56}$  & 5.42$_{\pm 6.44}$  &8.55$_{\pm 6.07}$ & 1.17$_{\pm 1.12}$    \\
& \multicolumn{1}{c|}{offline DQN (R)}      
& 4.40$_{\pm 1.57}$ & 10.55$_{\pm 5.50}$  &  2.41$_{\pm 0.92}$
& 0.97$_{\pm 0.47}$  & 5.59$_{\pm 2.84}$  &  3.52$_{\pm 1.38}$  \\
& \multicolumn{1}{c|}{offline DQN (E)}      
& 9.14$_{\pm 8.80}$ & 12.96$_{\pm 7.54}$  & 3.99 $_{\pm 1.18}$ 
& 2.75$_{\pm 0.20}$  & 10.54$_{\pm 7.98}$ & 3.63 $_{\pm 1.18}$ \\
% & \multicolumn{1}{c|}{offline RL (R)}      & 21.23 
% &
% & 21.24   &     & 20.54 &   \\
\cmidrule(l){2-8}
& \multicolumn{1}{c|}{LLM-based agent}      

& 16.72$_{\pm 2.26}$   & 20.63$_{\pm 2.55}$  & -
& - & - & -      \\
& \multicolumn{1}{c|}{offline DQN (LLM)}  
& 8.66$_{\pm 6.93}$  & 7.19$_{\pm 2.80}$  & 7.14$_{\pm 6.12}$ & 6.25$_{\pm 4.13}$ &9.99$_{\pm 4.10}$ & 4.19$_{\pm 3.09}$
\\
& \multicolumn{1}{c|}{offline DQN (MOE)}  
& \textbf{22.18$_{\pm 0.59}$}  & \textbf{20.84$_{\pm 2.63}$}   & \textbf{20.29$_{\pm 0.20}$} & \textbf{16.46 $_{\pm 4.03}$} &\textbf{17.38$_{\pm 0.63}$} & \textbf{4.69$_{\pm 2.54}$}
\\
\bottomrule
\end{tabular}

==> tables/prompt_pert_results.tex <==
\begin{tabular}{@{}cc|c|c|c|c@{}}
\toprule
\multicolumn{2}{c|}{Methods}                                                                                      & highway-fast             & highway             & highway-complex            & FetchSlide \\ \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{GPT3.5}}  & \multicolumn{1}{c|}{Teacher}      &  
&
&
&            \\
& \multicolumn{1}{c|}{online RL}      &  
&
&
&            \\
\cmidrule(l){2-6}
& \multicolumn{1}{c|}{offline DQN}  &\textbf{}
&\textbf{} 
&\textbf{}  &\textbf{}           
\\
& \multicolumn{1}{c|}{offline PPO}          
&
&
&
&
\\
& \multicolumn{1}{c|}{offline DDPG}
&      &
&
&
                       \\ \midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{GPT\-4}} & \multicolumn{1}{c|}{Teacher}    

&
&
&
&
\\
& \multicolumn{1}{c|}{online RL}      &  
&
&
&            \\
\cmidrule(l){2-6} 
& \multicolumn{1}{c|}{offline DQN} &
&

&
&
\\
& \multicolumn{1}{c|}{offline PPO}          
& 
&
&
&            \\
& \multicolumn{1}{c|}{offline DDPG}   
&
&
&
&           \\ \bottomrule
\end{tabular}

==> tables/safety_scores.tex <==
\begin{tabular}{@{}c|c|c|c|ccccc@{}}
\toprule
\multirow{2}{*}{Env}        & \multirow{2}{*}{$\epsilon$} & \multirow{2}{*}{Method} & \multirow{2}{*}{Clean} & \multicolumn{4}{c}{Attack Return}                      \\
&                          & &  & Uniform  & Gaussian & FGSM & PGD
\\ \midrule
\multirow{3}{*}{highway}  & \multirow{3}{*}{0.1}     
& online DQN & 14.38$_{\pm 1.57}$ 
& 16.68$_{\pm 6.78}$ 
&19.12$_{\pm 8.08}$ 
&3.24$_{\pm 2.29}$ 
&3.24$_{\pm 2.29}$
\\
& & offline DQN (LLM)      & 7.19$_{\pm 2.80}$
& 4.73$_{\pm 2.73}$
& 4.73$_{\pm 2.73}$
& 4.73$_{\pm 2.73}$
& 4.73$_{\pm 2.73}$
\\
& & robust offline DQN (MOE) 
& 20.84$_{\pm 2.63}$
& 6.18$_{\pm 3.47}$
& 6.18$_{\pm 3.47}$
& 6.18$_{\pm 3.47}$
& 6.18$_{\pm 3.47}$

\\
\midrule
\multirow{3}{*}{highway$-$medium} & \multirow{3}{*}{0.1}  
& online DQN & 5.42$_{\pm 6.44}$
& 3.61$_{\pm 1.11}$
& 3.12$_{\pm 1.17}$
& 3.01$_{\pm 1.29}$
& 3.01$_{\pm 1.29}$
\\
& 
& offline DQN (LLM) & 6.25$_{\pm 4.13}$
& 2.99$_{\pm 1.95}$
& 3.40$_{\pm 1.56}$
& 3.40$_{\pm 1.56}$
& 2.99$_{\pm 1.95}$

\\
& & robust offline DQN (MOE) & 16.46$_{\pm 4.03}$
& 4.63$_{\pm 4.07}$
& 4.63$_{\pm 4.07}$& 4.63$_{\pm 4.07}$& 4.63$_{\pm 4.07}$

\\
                            \midrule
\multirow{3}{*}{highway$-$hard}  & \multirow{3}{*}{0.1}     
& online DQN & 1.17$_{\pm 1.12}$
& 6.64$_{\pm 1.46}$
& 5.48$_{\pm 7.67}$
& 1.55$_{\pm 1.10}$
& 1.54$_{\pm 1.11}$
\\
&
& offline DQN (LLM)   &  4.19$_{\pm 3.09}$ & 2.55$_{\pm 2.10}$
& 2.22$_{\pm 1.99}$
& 2.22$_{\pm 1.99}$
& 1.88$_{\pm 2.18}$

\\

& & robust offline DQN (MOE) & 4.69$_{\pm 2.54}$

& 5.22$_{\pm 8.19}$
& 5.22$_{\pm 8.19}$
& 5.22$_{\pm 8.19}$
& 5.22$_{\pm 8.19}$


\\

\bottomrule
\end{tabular}
